Discriminative and Generative Transformer-based Models For Situation Entity Classification

We re-examine the situation entity (SE) classification task with varying amounts of available training data. We exploit a Transformer-based variational autoencoder to encode sentences into a lower dimensional latent space, which is used to generate the text and learn a SE classifier. Test set and cross-genre evaluations show that when training data is plentiful, the proposed model can improve over the previous discriminative state-of-the-art models. Our approach performs disproportionately better with smaller amounts of training data, but when faced with extremely small sets (4 instances per label), generative RNN methods outperform transformers. Our work provides guidance for future efforts on SE and semantic prediction tasks, and low-label training regimes.

==> additional_experiments.tex <==
\begin{table}[]
    \centering
    \scalebox{0.8}{        
    \begin{tabular}{l|cccc}
    \specialrule{.1em}{.05em}{.05em} 
    Genre     & Context Aware & Bert & Par Bert&LSTM Par Bert    &Humans \\ \hline
    blog      & 70.3       &\textbf{72.03}&74.14&72.68 & 72.9 \\
    email     & 71.5       &\textbf{73.84}&75.88&74.95 & 67.0 \\
    essays    & 64.1       &\textbf{66.99}&67.49&66.67 & 64.6 \\
    ficlets   & 68.8       &\textbf{75.14}&73.11&73.20 & 81.7 \\
    fiction   & 72.1       &\textbf{77.52}&75.42&77.28 & 76.7 \\ 
    gov-docs  & 68.9       &\textbf{72.52}&72.31&71.04 & 72.6\\
    jokes     & 75.0       &\textbf{77.11}&74.46&76.38 & 82.0\\
    journal   & 66.4       &\textbf{68.75}&68.81&70.68& 63.7\\
    letters   & 71.2       &\textbf{72.01}&75.64&74.07 & 68.0\\
    news      & 72.7       &\textbf{75.20}&74.58&76.42& 78.6\\
    technical & 60.5       &\textbf{61.72}&53.38&65.29&54.7\\
    travel    & 53.6       &\textbf{68.54}&54.74&58.28& 48.9\\
    wiki      & 60.6       &\textbf{63.04}&64.58&66.16& 69.2\\
    \specialrule{.1em}{.05em}{.05em} 
    \end{tabular}
    }
    \caption{Cross-genre Classification Results by Genre on the Training Set of MASC+Wiki.}
    \label{cross-genre result by genre}
\end{table}  

    \begin{table}[]
        \centering
        \begin{tabular}{l|ccc}
        \specialrule{.1em}{.05em}{.05em} 
        Genre     & Context Aware & Bert    &Humans \\ \hline
        blog      & 70.3       &\textbf{72.03} & 72.9 \\
        email     & 71.5       &\textbf{73.84} & 67.0 \\
        essays    & 64.1       &\textbf{66.99} & 64.6 \\
        ficlets   & 68.8       &\textbf{75.14}  & 81.7 \\
        fiction   & 72.1       &\textbf{77.52}  & 76.7 \\ 
        gov-docs  & 68.9       &\textbf{72.52} & 72.6\\
        jokes     & 75.0       &\textbf{77.11} & 82.0\\
        journal   & 66.4       &\textbf{68.75} & 63.7\\
        letters   & 71.2       &\textbf{72.01} & 68.0\\
        news      & 72.7       &\textbf{75.20} & 78.6\\
        technical & 60.5       &\textbf{61.72}& 54.7\\
        travel    & 53.6       &\textbf{68.54} & 48.9\\
        wiki      & 60.6       &\textbf{63.04} & 69.2\\
        \specialrule{.1em}{.05em}{.05em} 
        \end{tabular}
        \caption{Cross-genre Classification F-1 Scores by Genre on the Training Set of MASC+Wiki.}
        \label{cross-genre result by genre}
    \end{table}
    
    \begin{figure*}
    \centering
        \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/new/new_bert_lat_gen_f1.pdf}
        \caption{F1-macro}
        \label{fig:tiger}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/new/new_bert_lat_gen_acc.pdf}
        \caption{Accuracy}
        \label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/new/new_bert_lat_gen_prec.pdf}
        \caption{precision-macro}
        \label{fig:mouse}
    \end{subfigure}
\end{figure*}
\begin{table}[]
    \centering
    \scalebox{0.72}{        
    \begin{tabular}{l|ccccc}
    \specialrule{.1em}{.05em}{.05em} 
    Genre     & Context Aware & Bert & Par Bert & OptCls    &Humans \\ \hline
    blog      & 70.3       &{72.03}  & 74.14 & 72.37  & 72.9 \\
    email     & 71.5       &{73.84}  & 75.88 & 74.53  & 67.0 \\
    essays    & 64.1       &{66.99}  & 67.49 & 66.15  & 64.6 \\
    ficlets   & 68.8       &{75.14}  & 73.11 & 73.86  & 81.7 \\
    fiction   & 72.1       &{77.52}  & 75.42 & 78.99  & 76.7 \\ 
    gov-docs  & 68.9       &{72.52}  & 72.31 & 71.08  & 72.6 \\
    jokes     & 75.0       &{77.11}  & 74.46 & 76.73  & 82.0 \\
    journal   & 66.4       &{68.75}  & 68.81 & 71.96  & 63.7 \\
    letters   & 71.2       &{72.01}  & 75.64 & 71.93  & 68.0 \\
    news      & 72.7       &{75.20}  & 74.58 & 73.11  & 78.6 \\
    technical & 60.5       &{61.72}  & 53.38 & 62.72  & 54.7 \\
    travel    & 53.6       &{68.54}  & 54.74 & 58.18  & 48.9 \\
    wiki      & 60.6       &{63.04}  & 64.58 & 67.86  & 69.2 \\
    \specialrule{.1em}{.05em}{.05em} 
    \end{tabular}
    }
    \caption{Cross-genre Classification Results by Genre on the Training Set of MASC+Wiki.}
    \label{cross-genre-result-by-genre-sorted}
\end{table}  
% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/new/papers_code_bert_lat_gen_acc.pdf}
%   \caption{Original Code }
%   \label{fig:model}
% \end{figure*}
    % \begin{table}[]
    %     \centering
    %     \begin{tabular}{l|ccc}
    %     \specialrule{.1em}{.05em}{.05em} 
    %     Genre     & Context Aware & Bert    &Humans \\ \hline
    %     blog      & 70.3       &\textbf{72.03} & 72.9 \\
    %     email     & 71.5       &\textbf{73.84} & 67.0 \\
    %     essays    & 64.1       &\textbf{66.99} & 64.6 \\
    %     ficlets   & 68.8       &\textbf{75.14}  & 81.7 \\
    %     fiction   & 72.1       &\textbf{77.52}  & 76.7 \\ 
    %     gov-docs  & 68.9       &\textbf{72.52} & 72.6\\
    %     jokes     & 75.0       &\textbf{77.11} & 82.0\\
    %     journal   & 66.4       &\textbf{68.75} & 63.7\\
    %     letters   & 71.2       &\textbf{72.01} & 68.0\\
    %     news      & 72.7       &\textbf{75.20} & 78.6\\
    %     technical & 60.5       &\textbf{61.72}& 54.7\\
    %     travel    & 53.6       &\textbf{68.54} & 48.9\\
    %     wiki      & 60.6       &\textbf{63.04} & 69.2\\
    %     \specialrule{.1em}{.05em}{.05em} 
    %     \end{tabular}
    %     \caption{Cross-genre Classification F-1 Scores by Genre on the Training Set of MASC+Wiki.}
    %     \label{cross-genre result by genre}
    % \end{table}
    
    % \begin{figure}[t!]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/confusion/20_test_conf.pdf}
%   \caption{confusion matrix for test dataset. 20 samples}
%   \label{fig:conf_test_20}
% \end{figure}

% \label{sec:method}





There are other similar tasks such as aspectual class of verbs in context
\ForMR{This paragraph should be revised}
prediction~\citep{friedrich-palmer-2014-automatic}, fine-grained entity type classification (FETC) task~\citep{abhishek-etal-2017-fine}, entity mention classification to predict types from an entity type hierarchy~\citep{karn-etal-2017-end}, fine-grained information status determination which is basically a discourse entity classification task~\citep{rahman-ng-2012-learning}, and supervised identification of generic noun phrases~\citep{reiter-frank-2010-identifying} which can be employed to improve other tasks like knowledge acquisition.

==> questions.tex <==
Major concerns:
0- Why is this paper important? exciting?

1- Read the introduction: Does it motivate the reader to consider our approach? if not what should be added/revised/removed?

1A- Are the (scientific) contributions clear and do they go beyond "we obtain better performance?"

2- After reading the whole paper, do our experiments support all the claims we have made in the introduction?

3- What are the other experiments we could conduct that we have not done yet? we should mention them for future work or explain why we have ignored them.

4- Read the discussions in the experiments. Are they clear enough? are the comparisons fair? 

5- If an experiment is against our expectations, we should explain why? at least we should talk about our hypothesis that why this happened. 

6- We usually create a figure to explain our model. Is this figure informative and easy to grasp the idea behind our model structure?

7- Is the overall structure of the paper consistent?

8- Are the figures legible and accessible (avoiding color-blind color combinations, using multiple indicators to differentiate (e.g., shape+color, linetype+color))?

Minor concerns:
1- For each experiment if reformatting from a table to a bar-chart or any other combination can explain the points better, please mention that.  

2- Go through the equations, model descriptions. Sometimes we mistakenly use different notations for the same concept. If you find any mention that.
example: $\beta_{i,j}$ is defined as row $i$ and column $j$ in matrix $\beta$ but we mistakenly use $\beta_{i}^{j}$

3- Sentences with wrong grammar
